Doubly Inhomogeneous Reinforcement Learning

This paper studies reinforcement learning (RL) in doubly inhomogeneous environments under temporal non-stationarity and subject heterogeneity. In a number of applications, it is commonplace to encounter datasets generated by system dynamics that may change over time and population, challenging high-quality sequential decision making. Nonetheless, most existing RL solutions require either temporal stationarity or subject homogeneity, which would result in sub-optimal policies if both assumptions were violated. To address both challenges simultaneously, we propose an original algorithm to determine the ``best data chunks" that display similar dynamics over time and across individuals for policy learning, which alternates between most recent change point detection and cluster identification. Our method is general, and works with a wide range of clustering and change point detection algorithms. It is multiply robust in the sense that it takes multiple initial estimators as input and only requires one of them to be consistent. Moreover, by borrowing information over time and population, it allows us to detect weaker signals and has better convergence properties when compared to applying the clustering algorithm per time or the change point detection algorithm per subject. Empirically, we demonstrate the usefulness of our method through extensive simulations and a real data application.

==> latexmkrc <==
# HACK: this width seems to change with every compile, so
# latexmk runs latex too many times; ignore it
$hash_calc_ignore_pattern{'aux'} = 'statsocwidth';

# All the other default settings on Overleaf
# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

==> obsolete.tex <==
%as illustrated in Section \ref{sec:sim:synthetic:online}. %for online policy learning. 
%Nonetheless, 

%However, it remains challenging to identify the most recent ``best data segment of stationarity'' for each subject under heterogeneity.

%that %focus solely on either temporal non-stationarity or subject heterogeneity, 
    %implement the clustering algorithm per time point or the change point detection algorithm per subject, 

%Another example is the control of infectious disease such as the coronavirus disease 2019 (COVID-19) outbreak that had affected millions of people around the globe. Interests surged in RL to develop data-driven intervention policies to contain the spread of the virus \citep[see e.g.,][]{kompella2020reinforcement,wan2020multi}. However, the spread of COVID-19 is a doubly inhomogeneous process for several reasons. First, it is non-stationary over time due to the appearance of new variants. For instance, although lockdown measures were highly effective at the beginning of the pandemic, they might not be able to control the spread of more infectious variants. Second, the spread may also be heterogeneous across regions. For instance, regions where young people dominate the age structure, population density is low and the health insurance system is well-developed, have seen much better control over the disease spread than other regions \citep{vallee2022HeterogeneityCOVID19}. Finally, the timing difference of receiving COVID vaccines may induce both subject heterogeneity and temporal non-stationarity. Specifically, upon emergency use authorization of COVID vaccines, the spread of the virus was likely slower among people who were prioritized to receive the vaccines than those who were not. As the lower-prioritized groups received the vaccines later on, the spread of the virus among the two groups merged to the same rate. 

%Consider 
%Motivated by applications where rapid updating of the estimated policy is either not feasible or not necessary, %where the historical dataset is

 %The proposed algorithm is general, %and statistically efficient. Specifically, it %works as a wrapper framework that 
%and can take %as options 
%a wide range of off-the-shelf algorithms for clustering, change point detection and policy learning. %Additionally, it takes many possible initial change point estimators as input and only requires one of these initial estimators' overestimation errors to satisfy certain mild error rate conditions. We also discuss how to choose initial estimators to meet these conditions. 
 %Finally, we can apply any RL algorithm to the estimated data rectangles for policy learning and evaluation. Such an ``algorithm agnostic" property is particularly appealing in RL where new algorithms are emerging rapidly.

%For each of the $N$ subjects in the cohort, our objective lies in learning a warm-up policy to maximize their long-term rewards starting from time $T$, until a further change gets detected. As demonstrated in our numerical examples later, such a procedure can be repeatedly applied for updating the optimal policy at each current time as data accumulate. 

%A previous study \citep{li2022TestingStationarity} demonstrated that temporal nonstationarity of the optimal Q function might exist across different intern specialties, and neglecting this nonstationarity could result in suboptimal policies. However, in that work, heterogeneity was considered to exist only between specialties, not within them. The treatment effect of activity suggestions may shift from positive to negative, or vice versa, for different groups, indicating that treatment policies could benefit from adapting over time and identifying subgroups among the subjects. Ignoring potential nonstationarity and heterogeneity in treatment effects over time may lead to suboptimal policies, potentially overburdening subjects and resulting in app deletion and study dropouts.

%This observation underscores the importance of a time-adaptive and cluster-specific policy. Pooling all transition data collected over the 82 days and across all interns to learn a one-size-fits-all policy would obscure these changes and the inherent heterogeneity, leading to suboptimal outcomes.
%The Homogeneous method also detected a common change point at day 74 for all subjects, while the Stationary method failed to identify any cluster structure. Based on data from the first 82 days, the estimated average rewards for the four policies are as follows: Proposed (84537.83), DH/Stationary (82551.26), and Homogeneous (82259.69).
%The proposed policy is estimated to improve daily step counts by around 2,000 compared to other policies if used to guide activity suggestions, assuming the environment remains unchanged after day 82.

%Figures for other variables and results from the homogeneous method are provided in Supplement Section \ref{sec:sim:realIHS2020}.

%grouping observations with similar transition functions 

%We make a few remarks. (i) These two assumptions are satisfied in all the configurations introduced in Section \ref{sec:prelim:environment}. 
%(ii) LSE allows the change at time $T-\tau_i$ to be either an abrupt change, or a smooth change (e.g., the transition function changes smoothly until certain time and remains stationary afterwards), as shown in Supplemental Figure \ref{fig:abrupt_smooth_change}
% \ref{fig:dynamics_composite}(b)
%(iii) Together with LSE, LHE implies that within the $k$-th cluster, $p_{i,t}$ is a constant function of $(i,t)$ for any $i\in \mathcal{C}_k, T-\tau_i\le t\le T$. Once $\{\mathcal{C}_k\}_k$ and $\{\tau_i\}_i$ are identified, we can apply existing state-of-the-art RL algorithms to the data subset $\{O_{i,t}=(S_{i,t},A_{i,t},R_{i,t},S_{i,t+1}): i\in \mathcal{C}_k, t\ge  T-\tau_i \}$ with the same transition dynamics to derive the optimal warm-up policy for subjects within the $k$-th cluster. 
%(iv) We do not require the cluster membership to be known in advance, nor do we require to know the number of clusters $K$. (v) We do not impose any homogeneity assumption before the change point. In other words, for any two subjects $i_1$ and $i_2$ that belong to the same most recent cluster, the equality $p_{i_1,t_1}=p_{i_2,t_2}$ might not hold for $t_1< T-\tau_{i_1}$ or $t_2< T-\tau_{i_2}$. See e.g., the Merge and Merge \& Evolution examples in Figure \ref{fig:dynamics_illustration}. 
%\textbf{Data rectangles}. For a given $i$, let $\tau_{i,m}$ be the maximum of the collection of $\tau_i$’s that satisfy LSE. Then $T-\tau_{i,m}$ is the most recent change point for the $i$th subject. Equivalently, $\tau_{i,m}$ is the length of the largest most recent data interval of stationarity. 

% Given an initial set of estimators $\{\tau_{i}^0\}_i$ for $\{\tau_i^*\}_i$ and a given number of clusters $K$, we first apply the clustering algorithm to learn the cluster memberships and then apply the most recent change point detection algorithm to update the estimators for $\{\tau_i^*\}_i$. We next iterate this procedure a few times to obtain the final estimates $\{\widehat{\mathcal{C}}_k\}_k$ and $\{\widehat{\tau}_i^*\}_i$. Finally, for $1\le K\le K_{\max}$ integer $K_{\max}$ and a list of initial sets given by $\{\tau_i^{0,1}\}_i$, $\{\tau_i^{0,2}\}_i$, $\cdots$, $\{\tau_i^{0,J}\}_i$, we repeat this process $JK_{\max}$ times with different combinations of $\{\tau_{i}^0\}_i$ and $K$. This yields $JK_{\max}$ many %a list of 
% $(\{\widehat{\mathcal{C}}_k\}_k, \{\widehat{\tau}_i^*\}_i)$'s. We then select the %combination of $\{\widehat{\mathcal{C}}_k\}_k$ and $\{\widehat{\tau}_i^*\}_i$ 
% one that maximizes the following information criterion:

%We then show the proposed method is guaranteed to select the true number of clusters with a high probability.
%rate is also achievable when $K$ is over-specified and sample-splitting is employed to compute the final estimators (e.g., use half of data trajectories for clustering and the other half for change point detection).

%    \item According to Condition (ii) of Theorem \ref{thmrate}, the proposed doubly inhomogeneous algorithm only requires the signal $s_{cp}$ to be much larger than $N^{-1/2}T^{-1/4}\log(NT)$. This condition is required to guarantee the consistency of the proposed IC. 
    %$(NT)^{-1/2}$ up to some logarithmic factors for consistent change point detection. 
%    It is weaker than %the requirement of the Subject-wise algorithm: 
%    $s_{cp}\gg T^{-1/4}$ required by the Subject-wise algorithm, allowing us to detect weaker signals in settings with a diverging $N$.

%a singly inhomogeneous algorithm %, this rate is much faster than that obtained via 
%that applies the change point detection algorithm per subject: 

%(typically of the order $T^{-1}s_{cp}^{-2}$ up to some logarithmic factors), demonstrating the advantage of borrowing information across subjects. In addition, we only require $s_{cp}\gg (NT)^{-1/2}$ up to some logarithmic factors. This is weaker than requiring $s_{cp}\gg T^{-1/2}$, allowing us to detect weaker signals in settings with a diverging $N$. More importantly, when $N$ diverges at certain rate, the change point detection error can be smaller than $T^{-1}$, yielding an exactly zero change point error. This rate is generally impossible to achieve in settings with a single trajectory.

%Additionally, comparing the Time-wise algorithm against the Subject-wise algorithm, it can be seen that 

%For the Time-wise algorithm, this is because it only uses observations at the endpoint, and it is generally impossible to obtain a diminishing clustering error without repeated observations \citep{Marriott1975,ECTA11319}. In this sense, clustering is much more challenging compared to change point detection, because the latter handles observations with natural chronological order, although both problems are concerned with grouping observations with the same dynamics together. As for the Homogeneous algorithm, it is inconsistent as it ignores the nonstationary over time; see the proof of Theorem  \ref{thmregret} for details. 
%are closely related in the sense that both %

% When $K$ is over-specified, the \textit{over-clustering} error (e.g., an instance of subjects from several ground-truth clusters contained in the same cluster in the proposed clustering) equals exactly zero.  
%When $\{K_j\}_j$ contains the correct number of clusters, the IC is able to select the correct one.
%Moreover, we require the signal strength $s_{cl}$, the difference in the system dynamics across different clusters (see definition in Supplement Section \ref{sec:proof:auxiliary}) to be much larger than $T^{-1/2}$ up to some logarithmic factors. Notice that this condition is impossible to hold without repeated measurements (e.g., $T=1$). It suggests that borrowing information over time also allows us to largely relax the conditions on the signals. Nonetheless, with a finite $T$, it is generally impossible to obtain a diminishing clustering error even when $K$ is correctly specified \citep[see e.g.,][]{ECTA11319,Marriott1975}. In this case, clustering is much more challenging compared to change point detection, because the latter handles observations with natural chronological order. Both problems are closely related in the sense that both are concerned with grouping observations with the same dynamics together. 
% Nonetheless, change point detection is easier as observations are naturally ordered over time. 

%Finally, the proposed IC is able to correctly identify the number of clusters $K$ with high probability. 

%When taking multiple sets of initial estimators, we can vary $\varepsilon$ and use the proposed IC to adaptively select the initials.

%\begin{thm}\label{thmrateIC}
%    Suppose conditions in Theorem \ref{thmrate} are satisfied, %and $s_{cl}\gg K^0T^{-1/2} \sqrt{\log(NT)}$ where $K^0$ is the true number of clusters. 
    %Suppose that $K^0 \in \{K_j\}_j$.
    %Then under the IC in \eqref{eq:ic}, with probability $1-O(N^{-1}T^{-1})$, the proposed %algorithm 
%    the proposed IC selects the true number of clusters with probability approaching $1$.
    % with probability $1-O(N^{-1}T^{-1})$ for sufficiently large $C$.
%\end{thm}

\begin{comment}
We conduct numerical experiments to evaluate the finite sample performance of our method and compare it against existing solutions that ignore non-stationarity or heterogeneity. %Here we present fully 
Here we present the synthetic data results to illustrate the properties and utilities of the proposed algorithm. Results of semi-synthetic data mimicking the motivating IHS dataset are presented relegated to Supplement Section \ref{sec:sim:real:setting}.  Additional implementation details are provided in Supplement Section \ref{sec:sim:supp}\footnote{See also \url{https://anonymous.4open.science/r/DIRL-E1DE/} for a Python implementation of our method. }. 


%\subsection{Simulations}\label{sec:sim:synthetic}
\subsection{Offline Estimation and Consistency of the Information Criterion} \label{sec:sim:synthetic:offline}
\noindent \textbf{Data generating process}. We consider $K = 2$ clusters  each containing 25 subjects on the time interval $[0, T]$, where $T=50$. 
% Both clusters contain an abrupt change point in the state transition dynamics, at time $t = 35$ and 15, respectively. All subjects share the same reward function. The detailed data generating mechanism is provided in Supplement Section \ref{}
The state transition for the first cluster is $S_{it}=-0.5 S_{it-1}A_{it-1} + \cN(0, 0.25)$ before the change point $t = 35$, and is $S_{it}=0.5S_{it-1}A_{it-1}+\cN(0, 0.25)$ after change. The state transition for the second cluster is $S_{it}=0.5 S_{it-1}A_{it-1}+ \cN(0, 0.25)$ before the change point $t = 15$, and is $S_{it}=-0.5S_{it-1}A_{it-1}+ \cN(0, 0.25)$ after change. Here the actions $A_{it}$ are binary variables from Bernoulli$(0.5)$.
% Here, all $\epsilon_{it}$'s are i.i.d. standard normal random errors and all the actions are binary. 
The initial state $S_{i,0}$ is sampled from $\cN(0, 0.5)$. The reward function is defined the same for all subjects, given by $R_{it}=0.25 S_{it}^2A_{it}+4S_{it}$. We 
% fix $T=50$ and 
consider both abrupt and smooth changes (Supplement Section \ref{append:sec:implemetation} discusses how smooth changes are generated). 

\smallskip

\noindent \textbf{Initial estimators}. To demonstrate the consistency property of the proposed IC, we consider three sets of initial change points, including the oracle location ($\tau_i^0=\tau_i^*$ for any $i$), a random location ($T-\tau_1^0=\cdots=T-\tau_N^0=$ a uniformly randomly chosen location $\in [0,50)$) and no change point ($T-\tau_i^0=0$ for any $i$). We include the oracle location to demonstrate the performance of our algorithm with a perfect initialization. The latter two sets of change points do not generally satisfy the initial conditions in Theorem \ref{thmrate}. 
We anticipate the resulting final estimators $\{\widehat{\tau}_i^*\}_i$ will perform worse than those with the oracle initialization. In addition, we consider four different choices of $K$ from $\{1,2,3,4\}$. 
The constant $C$ in the IC \eqref{eq:ic} is set to 2. 

\smallskip

\noindent \textbf{Evaluation metrics}. We consider two evaluation criteria. To investigate the empirical performance of $\{\widehat{\tau}_i^*\}_i$, we define the change point detection error (CP error) as $\sum_{i=1}^N |\widehat{\tau}_i^* -\tau_i^*|(N\tau_i^*)^{-1}$. The larger the error, the worse the estimated change points. We also use the Adjusted Rand Index \citep[ARI,][]{hubert1985comparing} to measure the quality of estimated cluster memberships $\{\widehat{C}_k\}_k$. ARI which is a chance-corrected measure between $-1$ and $1$ with values near $1$ indicating higher degrees of concordance. 

\smallskip

\noindent \textbf{Results}.
% Figure \ref{fig:offline_err} shows change point detection results aggregated over 20 simulated datasets when we fix $K=2$ in the analysis. 
We first show that our IC is likely to select the initialization by the oracle change point locations when compared against the random initial location and the zero position. This demonstrates the robustness of our proposal with respect to the initial change points. We fix $K=2$ in this analysis. Results are reported in Figure \ref{fig:offline_err}, aggregated over 20 replications
% \ml{I probably forgot... Did we want to increase the number of replications?}. 
% The upper two panels and the lower two panels report the CP errors and the ARIs of the final estimators when taking the oracle location, the random location, the zero position or all of them (selected via the proposed IC) as initial change points. 
 The upper and lower panels display the CP errors and ARIs of the final estimators, respectively. These metrics were computed for different initial change point selections: the oracle location, the random location, the zero position, or a combination of these locations (selected through the proposed IC).
% The right two panels consider cases where we take the oracle location, the zero position or both as initials. 
It can be seen that results selected via our IC are very similar to those with the oracle location as the initial. Next, we show our IC is able to correctly determine the number of clusters. We fix $\tau_i^0=12$ for any $i$ and choose $K$ from $\{1,2,3,4\}$. Results are reported in Figure \ref{fig:offline_ic} in the Supplement, which shows that our IC is consistent in estimating the true number of clusters. 


\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{NeurIPS_2023/figures/offlineIC_cp2023-05-09.pdf}
    \vspace{-0.6in}
    \caption{Average CP error and ARI with different initial change point locations as well as the results where initials are chosen by the IC. Refer to Section \ref{sec:sim:synthetic:offline} for details.}
    \label{fig:offline_err}
\end{figure}

% \vspace{-0.25cm}



\subsection{Online Value Evaluation}\label{sec:sim:synthetic:online}
In this section, we demonstrate the utility of the proposed algorithm in policy learning. In each replication, we first simulate an offline dataset with $N=50$ and $T = 50$ from the same setting as in Section \ref{sec:sim:synthetic:offline}.  
Next, we apply our algorithm (with $\tau_i^0 = 5$ for any $i$, $K$ from $\{1,2,3,4\}$ and $C = 2$) to identify the most recent change points and cluster memberships, and then learn an optimal cluster-specific policy based on the estimated most recent data rectangles. For each of the 50 subjects, we combine the estimated optimal policy with the $\epsilon$-greedy algorithm ($\epsilon$ is fixed to $0.05$) for action selection and generate a new data batch for the next 25 time points, and apply our algorithm again to update the estimated optimal policy. Finally, we repeat this procedure to regularly update the estimated optimal policy assuming the online data arrive in batches every 25 time points, until we reach the terminal time $250$. In the data generating process, the two clusters are allowed to merge, split or switch whereas the potential change points follow a Poisson process. See Supplement Section \ref{sec:sim:syn:evaluation} for more details about the setting and the policy learning algorithm. We compute the average reward (i.e., value) aggregated over time (from $t=51$ to $250$) and population following the proposed policies. We compare this value against the values obtained using the following policies: (i) an oracle policy learned as if the oracle $\{\tau_i^*\}_i$ and $\{\mathcal{C}_k\}_k$ were known; (ii) a doubly homogeneous (DH) policy learned based on all historical data, ignoring non-stationarity or heterogeneity; (iii) a homogeneous policy learned based on the estimated most recent change points only, ignoring heterogeneity; (iv) a stationary policy learned based on the estimated cluster memberships only, ignoring non-stationarity. 

Figure \ref{fig:online_avr} reports the value of the proposed policy and the baseline policies, aggregated over 20 replications. 
The proposed policy achieves slightly lower but similar value to the oracle policy. To the contrary, the other policies produce significantly smaller values, demonstrating the danger of ignoring either inhomogeneity. Figure \ref{fig:same_value} in the Supplement reports the average value in a different setting where the optimal policy is agnostic to change points or cluster memberships.
% the two clusters possess different dynamics but share the same optimal policy. 
In this case, the doubly homogeneous (DH) policy achieves the best performance as it utilises a larger amount of relevant data for policy learning. Meanwhile, all other policies achieve comparable performance. 


\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{figures/diff_av_value2023-04-24.pdf}
\vspace{-0.1in}
\caption{Boxplot of the expected returns under the proposed policy and other baseline policies that either ignore non-stationarity or heterogeneity. Refer to Section \ref{sec:sim:synthetic:online} for details.}
\label{fig:online_avr}
\end{figure}
\end{comment}
% \subsection{Real Data-based Simulation}\label{sec:sim:real}
% To mimic the motivating IHS study, we simulate a dataset with $K = 3$ clusters, each containing $50$ subjects over $T = 26$ time points. 
% Our goal is to estimate an optimal treatment policy to improve these interns' long-term physical activity levels. The state vector comprises three variables to mimic the actual IHS study: the square root of weekly step count, the cubic root of weekly sleep minutes, and the average weekly mood score. 
% The actions are binary; $A_{it} = 1$ means the subject is randomized to receive activity messages at time $t$ whereas $A_{it} = 0$ means any other types of messages or no messages at all. Prior work found that three clusters are likely to encounter different numbers of change points \citep{li2022TestingStationarity}. To mimic the real dataset setup, we similarly assume that cluster 1 sees one change point, and cluster 3 sees no change point throughout the study.
% See Supplement Section \ref{sec:sim:real:setting} for the true transition functions for the three subjects clusters. The simulated dynamics resemble a composite system configuration consisting of Evolution $\&$ Constancy, as illustrated in Figure \ref{fig:dynamics_illustration}. 
% We further consider three different scenarios with strong, moderate, and weak signals, by varying the magnitude of the treatment effect on the future state. We use the proposed IC to choose $K$ from $\{2,3,4\}$ and to select $\tau^0=\tau_1^0=\cdots=\tau_N^0$ from $\{15, 20\}$.

% Figure \ref{fig:sim:offline:real} depicts the CP errors and the ARIs of the proposed estimators under different signal strengths. With strong signals, the CP errors equal zero and the ARIs equal 1 in most cases. This is consistent with our theoretical findings. With weak signals, the CP errors are close to 0.2 whereas the ARIs are slightly larger than 0.5. With moderate signals, both evaluation criteria vary a lot across different replications due to the uncertainty in $K$ selection. When the proposed IC correctly selects $K$, the results are similar to those under strong signals, or otherwise similar to those under weak signals. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/real_boxplot_simresult_C0.pdf}
%     \caption{The CP error and the ARI of the proposed method in detecting change points and identifying clusters with three different signal strengths. Refer to Section 5.2 for details.}
%     \label{fig:sim:offline:real}
% \end{figure}

% \begin{figure}
% \centering
% \begin{minipage}[c]{\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/real_boxplot_simresult.pdf}
% \end{minipage}
% \vspace{0.2cm}
% \begin{minipage}[c]{\textwidth}
%     \centering
%     (a) Offline results: CP errors and ARIs of the proposed method.
% \end{minipage}
% \begin{minipage}[c]{\textwidth}
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/real_optvalue_online_discounted.pdf} 
% \end{minipage}
% \begin{minipage}[c]{\textwidth}
%     \centering
%     (b) Online results: discounted rewards for $\gamma = 0.9$.
% \end{minipage}
% \vspace{-0.15in}
% \caption{Semi-synthetic data simulation results under three different signal strengths.}
% \label{fig:sim:offline:real}
% \end{figure}

%{\color{blue} For a singly inhomogeneous method, either the change points or the clusters cannot be identified.}

%estimate an optimal warm-up treatment policy at the current time $T$ to improve these interns' long-term physical activity levels.
%There are two most recent data segments where the dynamics are doubly homogeneous in the offline dataset, based on the previously described data generating process. The first segment consists of transition data for $i \in [1, 20]$ and $t \in [50, 99]$. The second segment consists of transition data for $i \in [21, 60]$ and $t \in [50, 99]$.
  %When applying the proposed algorithm to the simulated data, we used the proposed IC to select the best estimation results, by choosing $K$ from $\{1,2,3,4\}$.  %Additional details of the system dynamics and implementation are provided in Supplement Section \ref{sec:sim:real:additional}.

% \smallskip

%We compared the change points and clusters detected by the proposed method against the following approaches: (i) Time-wise Cluster Detection (TCD); (ii) Subject-wise Change Point Detection (TCPD); (iii) a homogeneous method that detects universal change points for all trajectories; and (iv) a stationary method that detects clusters based on time points across the entire horizon.}
% \smallskip

\begin{comment}
\begin{table}[h!]
    \centering
    \caption{Offline restuls: Change Point Error and ARI of the proposed method.}\label{tab:semisyn offline}
    \begin{tabular}{lcc}
        \toprule
        Signal strength & Change Point Error & ARI \\
        \midrule
        Strong & 0.16 (0.01) & 1.00 (0.00) 
        % Strong & 0.158 (0.008) & 1.000 (0.000) 
        \\
        Moderate & 0.42 (0.01) & 1.00 (0.00) 
        % Moderate & 0.420 (0.014) & 1.000 (0.000)
        \\
        Weak & 0.50 (0.00) & 0.74 (0.07) 
        % Weak & 0.495 (0.000) & 0.742 (0.069) 
        \\
        \bottomrule
    \end{tabular}
\end{table}
\end{comment}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/real_boxplot_simresult_C0.pdf}
%     \caption{Semi-synthetic data simulation results: the CP errors and the ARIs of the proposed method under three different signal strengths.}
%     \label{fig:sim:offline:real}
% \end{figure}



%among the interns around day 70: one subgroup increases sleep duration, while the other decreases. This heterogeneous response indicates that the interns likely faced different environmental factors after day 70, possibly due to events such as exams or shift work, implying that different activity policies may be beneficial for each cluster.

% The difference in the cumulative discounted rewards can be found in Supplement Section \ref{sec:sim:real:evaluation:additional}.
% {\color{red}Figure \ref{fig:same_value} in the Supplement reports a different setting where the optimal policy is agnostic to change points or cluster memberships.
% In this case, the doubly homogeneous (DH) policy achieves the best performance as it utilises a larger amount of relevant data for policy learning, while all other policies achieve comparable performances. }



% \begin{table}[htbp]
%     \centering
%     \caption{Online results: average reward}\label{tab:semisyn online average}
%     \begin{tabular}{lccc}
%         \toprule
%         Policy & Strong & Moderate & Weak \\
%         \midrule
%         Proposed-Oracle & -0.0051 (0.0025) & -0.0013 (0.0008) & -0.0027 (0.0007) \\
%         Proposed-DH & 0.0090 (0.0026) & 0.0065 (0.0005) & 0.0024 (0.0007) \\
%         Proposed-Homogeneous & 0.0170 (0.0031) & 0.0071 (0.0006) & 0.0029 (0.0009) \\
%         Proposed-Stationary & 0.0063 (0.0022) & 0.0046 (0.0008) & 0.0008 (0.0005) \\
%         \bottomrule
%     \end{tabular}
% \end{table}

\begin{comment}
Figure \ref{fig:realdata:proposed_sleep_cpcluster} shows the sleep trajectories for each cluster detected by the proposed method, along with cluster-specific change points for $T_{train}=82$. The proposed method identified two clusters, comprising 520 and 504 subjects, with change points occurring at days 70 and 74, respectively. The red vertical lines mark these change points, while the green and yellow horizontal lines indicate the mean values before and after the change points.
Notably, there is a significant increase in the mean step count for the first cluster after day 70, while the second cluster experiences a decrease after day 74. This divergence suggests the existence of two subgroups among the interns around day 70: one subgroup increases sleep duration, while the other decreases. This heterogeneous response indicates that the interns likely faced different environmental factors after day 70, possibly due to events such as exams or shift work, implying that different activity policies may be beneficial for each cluster.
This observation underscores the importance of a time-adaptive and cluster-specific policy. Pooling all transition data collected over the 82 days and across all interns to learn a one-size-fits-all policy would obscure these changes and the inherent heterogeneity, leading to suboptimal outcomes.
The Homogeneous method also detected a common change point at day 74 for all subjects, while the Stationary method failed to identify any cluster structure. Based on data from the first 82 days, the estimated average rewards for the four policies are as follows: Proposed (84537.83), DH/Stationary (82551.26), and Homogeneous (82259.69).
The proposed policy is estimated to improve daily step counts by around 2,000 compared to other policies if used to guide activity suggestions, assuming the environment remains unchanged after day 82.
Although the Homogeneous method detected a change point at day 74, the policy learned from data after this change point has the lowest estimated value. This is likely because the environment faced by the interns changed in different ways after day 74, as illustrated in Figure \ref{fig:realdata:proposed_sleep_cpcluster}.
We further fit two linear regression models using the data for the first and second clusters after their respective change points and found that the two clusters may indeed have different effects from activity suggestions. Specifically, the linear regression coefficient of the action for one cluster is positive, while it is negative for the other, which might indicate differing responses to the activity suggestions between the clusters (see \ref{sec:sim:real:setting} for the fitted coefficients).
Figures for other variables and results from the homogeneous method are provided in Supplement Section \ref{sec:sim:realIHS2020}.
\end{comment}

% The stationary method, which fails to identify any cluster structures, performs similarly to the doubly homogeneous method, further underscoring the advantage of the proposed approach.








% \begin{table}[ht]
%     \begin{minipage}[b]{0.45\linewidth}
%         \centering
%         \caption{Cross-validated OPE values.}
%         \begin{tabular}{|c|c|}
%             \hline
%             Method & OPE value \\
%             \hline
%             Proposed & -0.0594 \\
%             Homogeneous & -0.0977 \\
%             Stationary & -0.177 \\
%             DH & -0.177 \\
%             \hline
%         \end{tabular}
%         \label{tab:realdata_opevalues}
%     \end{minipage}
%     \hspace{0.05\linewidth}
%     \begin{minipage}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{jrssb/figures/proposed_step_cluster_changepoints.png} 
%         \caption{Change points and clusters detected by the proposed method}
%         \label{fig:realdata:proposed_step_cpcluster}
%     \end{minipage}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Discussion}
%This paper studies reinforcement learning (RL) in doubly inhomogeneous environments. The proposed algorithm is robust not only to the hostility of the environment (e.g., temporal non-stationarity and subject heterogeneity), but to the choice of the initial estimators as well, and is thus safe to use in practice. In applications where learning optimal policies to maximize the expectation of the returns must ensure system performance and/or respect safety constraints (e.g., preventing an action that may lead to user disengagement from mobile prompts), safe RL \citep{garcia2015comprehensive,brunke2022safe,gu2022review} is critical.  

\begin{comment}
To handle double inhomogeneity, we assume the system is locally stationary and homogeneous, and employ change point detection and clustering to group observations with similar transition dynamics together for policy learning. More generally, one may assume the existence of certain subject-specific and time-specific latent factors (denoted by $\{v_i\}_i$ and $\{u_t\}_t$, respectively) such that the transition function is doubly homogeneous if these factors were known, i.e., $p_{i,t}(\bullet|a,s)=p(\bullet|a,s,v_i,u_t)$ for any $a,s,u,t$. Such an approach is similar to factor modelling that is widely studied in the economics literature. Nonetheless, it remains unclear how to estimate these latent factors in our setting. We leave it for future research. 

In this paper, we have not considered the important role of individual-level covariates or features to partly explain potential between-subject heterogeneity. Additional work is warranted to place individuals with more similar covariates in the same cluster via model-based clustering approaches such as product partition models \citep{muller2011product}. Similarly, covariates may impact the change points, which can be readily addressed by including the covariates into the state variables. Nevertheless, the present paper puts forth a formal theoretical framework to incorporate this additional information and provides an exploratory tool to discover subject clusters for additional considerations of potential causes of inhomogeneity and guide feature discovery. 
\end{comment}



%presents the average OPE values from $T_{train}=62$ to $T_{train}=82$ for policies obtained using different methods. 
%highlighting the potential benefits of employing a cluster-tailored policy with updated data to improve the long-term health conditions of the interns.
%On average, the optimal cluster-specific policy, estimated using data after the detected change point,

%We compared the average reward obtained by the proposed policy against the following policies: (i) an oracle policy learned as if the oracle $\{\tau_i^*\}_i$ and $\{\mathcal{C}_k\}_k$ were known; (ii) a doubly homogeneous (DH) policy learned using all historical data, ignoring non-stationarity or heterogeneity; (iii) a homogeneous policy learned using the estimated most recent change points only, ignoring heterogeneity; (iv) a stationary policy learned using the estimated cluster memberships only, ignoring non-stationarity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \begin{figure}[t]
%     \centering 
%     \includegraphics[width=0.3\textwidth]{./figures/dynamics_different_cp}
%     \vspace{-0.1in}
%     \singlespacing
%     \caption{Illustration of different change points in the same subject clusters. Subjects 1 and 2 evolve to a new shared dynamic at time points $t_1^*$ and $t_2^*$, respectively. In the cluster that involves the two subjects, the most recent change point is $T - t_2^*$. The most recent change point for the cluster involving subject 3 is $T - t_3^*$. }
%     \label{fig:dynamics_different_cp}
% \end{figure}

%In the statistics literature, RL is closely related to a line of research on dynamic treatment regimes (DTRs). We refer the reader to \cite{tsiatis2019dynamic} and \cite{kosorok2019precision} for overviews. Nonetheless, most proposals on DTRs are motivated by applications in precision medicine with a few treatment stages. 
%Recently, there is a growing interest in developing offline RL algorithms \citep[see e.g.,][]{kumar2019stabilizing,levine2020offline,yu2020mopo,jin2021pessimism,xie2021bellman,yin2021towards,baipessimistic,shi2022pessimistic,ueharapessimistic,zhou2023optimizing}. %in the statistics literature. See e.g. \cite{Ertefaie2018,luckett2020estimating,%liao2019off,ramprasad2021online,liao2020batch,shi2020statistical,zhou2021estimating}. 
%\subsection{Motivation}






% \section*{References}
% References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for the references. Any choice of citation style is acceptable as long as you are consistent. It is permissible to reduce the font size to \verb+small+ (9 point) when listing the references. Note that the Reference section does not count towards the page limit.
% \medskip

% {
% \small


% [1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
% connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
% (eds.), {\it Advances in Neural Information Processing Systems 7},
% pp.\ 609--616. Cambridge, MA: MIT Press.


% [2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
%   Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
% TELOS/Springer--Verlag.


% [3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
% recall at excitatory recurrent synapses and cholinergic modulation in rat
% hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
% }

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\bibliographystyle{IEEEtran} %agsm
